Some remarks on discrete and semi-discrete transparent boundary conditions for solving the time-dependent Schr\"odinger equation on the half-axis

We consider the generalized time-dependent Schr\"odinger equation on the half-axis and a broad family of finite-difference schemes with the discrete transparent boundary conditions (TBCs) to solve it. We first rewrite the discrete TBCs in a simplified form explicit in space step $h$. Next, for a selected scheme of the family, we discover that the discrete convolution in time in the discrete TBC does not depend on $h$ and, moreover, it coincides with the corresponding convolution in the semi-discrete TBC rewritten similarly. This allows us to prove the bound for the difference between the kernels of the discrete convolutions in the discrete and semi-discrete TBCs (for the first time). Numerical experiments on replacing the discrete TBC convolutions by the semi-discrete one exhibit truly small absolute errors though not relative ones in general. The suitable discretization in space of the semi-discrete TBC for the higher-order Numerov scheme is also discussed.

==> table.tex <==
\pgfplotstableset{%
    empty cells with={--}, % replace empty cells with '--'
    every head row/.style={%
        before row=\toprule, after row=\midrule
    },
%    every even row/.style={%
%        before row={\rowcolor[gray]{0.9}}
%    },
    every last row/.style={%
        after row=\bottomrule
    },
    col sep=semicolon,
    1000 sep={\,},
    dec sep align,
    sci zerofill,
}
\pgfplotstableread{data/EX01_DTBC_J.csv}\dataJ
\pgfplotstableread{data/EX01_DTBC_M.csv}\dataM
\pgfplotstableread{data/EX01_SDTBC_J.csv}\dataSJ
\pgfplotstableread{data/EX01_SDTBC_M.csv}\dataSM
\pgfplotstableread{data/EX01_DTBCvsSDTBC_J.csv}\dataDSJ
\pgfplotstableread{data/EX01_DTBCvsSDTBC_M.csv}\dataDSM
\pgfplotstableread{data/EX01_DTBCvsSDTBC+FEM_J.csv}\dataDSFJ
\pgfplotstableread{data/EX01_DTBCvsSDTBC+FEM_M.csv}\dataDSFM
%
\par\pgfplotstabletypeset[%
%    row predicate/.code={%
%        \pgfplotstablegetelem{#1}{[index]1}\of{\data}
%        \ifnum\pgfplotsretval=1200
%            \pgfplotstablegetelem{#1}{[index]2}\of{\data}
%            \ifnum\pgfplotsretval=128
%                \relax
%            \else
%                \pgfplotstableuserowfalse
%            \fi
%        \else
%            \pgfplotstableuserowfalse
%        \fi
%    },
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={11}},
    columns={[index]0,[index]4,rLa,[index]3,rCa,[index]6,rLr,[index]5,rCr},%,[index]7,ct
    columns/0/.style={column name=$J$,},%0
    columns/1/.style={column name=$M$,},%1
    columns/2/.style={column name=$K$,},%2
    columns/3/.style={column name=$E_C$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh})}$
    columns/4/.style={column name=$E_{L^2}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh}}$
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh}),\,{\rm rel}}$
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh},\,{\rm rel}}$
    columns/7/.style={column name=$E_C(M)$,},
    columns/8/.style={column name=$E_{L^2}(M)$,},
    columns/9/.style={column name=$E_{C,\,{\rm rel}}(M)$,},
    columns/10/.style={column name=$E_{L^2,\,{\rm rel}}(M)$,},
%    columns/11/.style={column name=$T\,\,{\rm sec.}$, int trunc,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=EX01_DTBC_J.tex
]{\dataJ}
%
\vskip1cm
\par\pgfplotstabletypeset[%
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={11}},
    columns={[index]1,[index]4,rLa,[index]3,rCa,[index]6,rLr,[index]5,rCr},%,[index]7,ct
    columns/0/.style={column name=$J$,},
    columns/1/.style={column name=$M$,},
    columns/2/.style={column name=$K$,},
    columns/3/.style={column name=$E_{C}$,},
    columns/4/.style={column name=$E_{L^2}$,},
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},
    columns/7/.style={column name=$E_C(M)$,},
    columns/8/.style={column name=$E_{L^2}(M)$,},
    columns/9/.style={column name=$E_{C,\,{\rm rel}}(M)$,},
    columns/10/.style={column name=$E_{L^2,\,{\rm rel}}(M)$,},
%    columns/11/.style={column name=$T\,\,{\rm sec.}$, int trunc,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=EX01_DTBC_M.tex
]{\dataM}

\par\pgfplotstabletypeset[%
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={11}},
    columns={[index]0,[index]4,rLa,[index]3,rCa,[index]6,rLr,[index]5,rCr},%,[index]7,ct
    columns/0/.style={column name=$J$,},%0
    columns/1/.style={column name=$M$,},%1
    columns/2/.style={column name=$K$,},%2
    columns/3/.style={column name=$E_C$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh})}$
    columns/4/.style={column name=$E_{L^2}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh}}$
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh}),\,{\rm rel}}$
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh},\,{\rm rel}}$
    columns/7/.style={column name=$E_C(M)$,},
    columns/8/.style={column name=$E_{L^2}(M)$,},
    columns/9/.style={column name=$E_{C,\,{\rm rel}}(M)$,},
    columns/10/.style={column name=$E_{L^2,\,{\rm rel}}(M)$,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=EX01_SDTBC_J.tex
]{\dataSJ}
%
\vskip1cm
\par\pgfplotstabletypeset[%
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={11}},
    columns={[index]1,[index]4,rLa,[index]3,rCa,[index]6,rLr,[index]5,rCr},%,[index]7,ct
    columns/0/.style={column name=$J$,},
    columns/1/.style={column name=$M$,},
    columns/2/.style={column name=$K$,},
    columns/3/.style={column name=$E_{C}$,},
    columns/4/.style={column name=$E_{L^2}$,},
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},
    columns/7/.style={column name=$E_C(M)$,},
    columns/8/.style={column name=$E_{L^2}(M)$,},
    columns/9/.style={column name=$E_{C,\,{\rm rel}}(M)$,},
    columns/10/.style={column name=$E_{L^2,\,{\rm rel}}(M)$,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=EX01_SDTBC_M.tex
]{\dataSM}

\par\pgfplotstabletypeset[%
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={11}},
    columns={[index]0,[index]4,rLa,[index]3,rCa,[index]6,rLr,[index]5,rCr},%,[index]7,ct
    columns/0/.style={column name=$J$,},%0
    columns/1/.style={column name=$M$,},%1
    columns/2/.style={column name=$K$,},%2
    columns/3/.style={column name=$E_C$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh})}$
    columns/4/.style={column name=$E_{L^2}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh}}$
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh}),\,{\rm rel}}$
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh},\,{\rm rel}}$
    columns/7/.style={column name=$E_C(M)$,},
    columns/8/.style={column name=$E_{L^2}(M)$,},
    columns/9/.style={column name=$E_{C,\,{\rm rel}}(M)$,},
    columns/10/.style={column name=$E_{L^2,\,{\rm rel}}(M)$,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=EX01_DTBCvsSDTBC_J.tex
]{\dataDSJ}
%
\vskip1cm
\par\pgfplotstabletypeset[%
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={11}},
    columns={[index]1,[index]4,rLa,[index]3,rCa,[index]6,rLr,[index]5,rCr},%,[index]7,ct
    columns/0/.style={column name=$J$,},
    columns/1/.style={column name=$M$,},
    columns/2/.style={column name=$K$,},
    columns/3/.style={column name=$E_{C}$,},
    columns/4/.style={column name=$E_{L^2}$,},
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},
    columns/7/.style={column name=$E_C(M)$,},
    columns/8/.style={column name=$E_{L^2}(M)$,},
    columns/9/.style={column name=$E_{C,\,{\rm rel}}(M)$,},
    columns/10/.style={column name=$E_{L^2,\,{\rm rel}}(M)$,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=EX01_DTBCvsSDTBC_M.tex
]{\dataDSM} 

\par\pgfplotstabletypeset[%
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={11}},
    columns={[index]0,[index]4,rLa,[index]3,rCa,[index]6,rLr,[index]5,rCr},%,[index]7,ct
    columns/0/.style={column name=$J$,},%0
    columns/1/.style={column name=$M$,},%1
    columns/2/.style={column name=$K$,},%2
    columns/3/.style={column name=$E_C$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh})}$
    columns/4/.style={column name=$E_{L^2}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh}}$
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},    %$\max\limits_{1\leq m\leq M}\|e^m\|_{C(\overline{\omega}_{\bh}),\,{\rm rel}}$
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},  %$\max\limits_{1\leq m\leq M}\|e^m\|_{\widetilde{\omega}_{\bh},\,{\rm rel}}$
    columns/7/.style={column name=$E_C(M)$,},
    columns/8/.style={column name=$E_{L^2}(M)$,},
    columns/9/.style={column name=$E_{C,\,{\rm rel}}(M)$,},
    columns/10/.style={column name=$E_{L^2,\,{\rm rel}}(M)$,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=EX01_DTBCvsSDTBC+FEM_J.tex
]{\dataDSFJ}
%
\vskip1cm
\par\pgfplotstabletypeset[%
    create on use/rCa/.style={create col/quotient={3}},
    create on use/rLa/.style={create col/quotient={4}},
    create on use/rCr/.style={create col/quotient={5}},
    create on use/rLr/.style={create col/quotient={6}},
    create on use/ct/.style={create col/iquotient={11}},
    columns={[index]1,[index]4,rLa,[index]3,rCa,[index]6,rLr,[index]5,rCr},%,[index]7,ct
    columns/0/.style={column name=$J$,},
    columns/1/.style={column name=$M$,},
    columns/2/.style={column name=$K$,},
    columns/3/.style={column name=$E_{C}$,},
    columns/4/.style={column name=$E_{L^2}$,},
    columns/5/.style={column name=$E_{C,\,{\rm rel}}$,},
    columns/6/.style={column name=$E_{L^2,\,{\rm rel}}$,},
    columns/7/.style={column name=$E_C(M)$,},
    columns/8/.style={column name=$E_{L^2}(M)$,},
    columns/9/.style={column name=$E_{C,\,{\rm rel}}(M)$,},
    columns/10/.style={column name=$E_{L^2,\,{\rm rel}}(M)$,},
    columns/rCa/.style={column name=$R_{C}$,},
    columns/rLa/.style={column name=$R_{L^2}$,},
    columns/rCr/.style={column name=$R_{C,\,{\rm rel}}$,},
    columns/rLr/.style={column name=$R_{L^2,\,{\rm rel}}$,},
    columns/ct/.style={column name=$R_{\rm time}$,},
    outfile=EX01_DTBCvsSDTBC+FEM_M.tex
]{\dataDSFM} 
